Browser-based Analysis of Web Framework Applications

Although web applications evolved to mature solutions providing sophisticated user experience, they also became complex for the same reason. Complexity primarily affects the server-side generation of dynamic pages as they are aggregated from multiple sources and as there are lots of possible processing paths depending on parameters. Browser-based tests are an adequate instrument to detect errors within generated web pages considering the server-side process and path complexity a black box. However, these tests do not detect the cause of an error which has to be located manually instead. This paper proposes to generate metadata on the paths and parts involved during server-side processing to facilitate backtracking origins of detected errors at development time. While there are several possible points of interest to observe for backtracking, this paper focuses user interface components of web frameworks.

==> eptcsdata.tex <==
\providecommand{\firstpage}{51}
\providecommand{\publicationstatus}{Sala\"un, Fu, and Hall\'e (Eds.): Fourth International Workshop\\
on Testing, Analysis and Verification of Web Software\\
EPTCS 35, 2010, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.35.5}{10.4204/EPTCS.35.5}}

